Accounting for Seasonality in Extreme Sea Level Estimation

Reliable estimates of sea level return levels are crucial for coastal flooding risk assessments and for coastal flood defence design. We describe a novel method for estimating extreme sea levels that is the first to capture seasonality, interannual variations and longer term changes. We use a joint probabilities method, with skew surge and peak tide as two sea level components. The tidal regime is predictable but skew surges are stochastic. We present a statistical model for skew surges, where the main body of the distribution is modelled empirically whilst a non-stationary generalised Pareto distribution (GPD) is used for the upper tail. We capture within-year seasonality by introducing a daily covariate to the GPD model and allowing the distribution of peak tides to change over months and years. Skew surge-peak tide dependence is accounted for via a tidal covariate in the GPD model and we adjust for skew surge temporal dependence through the subasymptotic extremal index. We incorporate spatial prior information in our GPD model to reduce the uncertainty associated with the highest return level estimates. Our results are an improvement on current return level estimates, with previous methods typically underestimating. We illustrate our method at four UK tide gauges.

==> Acc_mt_seasonality.tex <==
%\textcolor{red}{Jon said to add this paragraph here?} In the UK, the tidal regime is semi-diurnal because a full tidal cycle of one high tide and one low tide takes approximately 12 hours 25 minutes. The timing and magnitude of low and high tides varies across the UK coastline. The range of semi-diurnal tides typically follow a 14 day cycle, where the greatest ranges are observed when the Sun and Moon are in line with the Earth at full or new Moon, this is known as spring tide. Periods of smaller tidal ranges are called neap tides, when the sun and moon are perpendicular to the Earth. 

So far, we have assumed within-year stationarity of tides and therefore selected sequences $\{X_{j_i}^{(s)}\}$ of consecutive peak tides starting from any point within the time series. We have also assumed the tidal regime is the same across years, but interannual variations exist. In this section, we describe how to account for these features.

To account for within-year variations, we simply choose our contiguous peak tide samples from the month of interest, denoted $\{X_{i}^{(j)}\}_{i=1}^{T_j}$. To account for interannual variations, we begin by deriving the distribution of the monthly maxima for a fixed year. We adapt our notation so that we know the year, as well as the month, of observation. We denote the year by $k=1,\ldots,K$ for $K$ total years of observation. Then the tidal sample is taken from the month and year of interest, $X_{i}^{(j,k)}$ for $i=1,\ldots,T_{j}^{(k)}$ where $T_j^{(k)}$ reflects that the number of tidal cycles changes for a fixed month across years because the timing of the first cycle in the month can vary annually. Assuming skew surges are independent and incorporating the seasonal model from equation \eqref{final_ss_model}, we write the distribution of the monthly maxima in a given year $k$, $M_j^{(k)}$, as
\begin{equation}
    \mathbb{P}(M_j^{(k)}\leq{z})=\prod\limits_{{i}=1}^{T^{(k)}_j}\mathbb{P}(Y_{i}^{(j)}\leq{z- X_{i}^{(j,k)}})=\prod\limits_{{i}=1}^{T^{(k)}_j}F_Y^{(d,j)}(z- X_{i}^{(j,k)}).
\end{equation}

Similarly, to find the distribution of the annual maxima, we first find the annual maxima distribution for a fixed year $k$, denoted $M^{(k)}$. This is given by \begin{equation}
    \mathbb{P}(M^{(k)}\leq{z})=\prod\limits_{j=1}^{12}\mathbb{P}(M_j^{(k)}\leq{z})=\prod\limits_{j=1}^{12}\Bigg(\prod\limits_{{i}=1}^{T^{(k)}_j}F_Y^{(d,j)}(z- X_{i}^{(j,k)})\Bigg)\label{annmax_seasonality_givenyr}.
\end{equation}

Then we assume each observed annual tidal regime has an equal probability of occurrence and average over all possibilities, we write the distribution an arbitrarily selected monthly maxima $M_j$ as\begin{equation}
    \mathbb{P}(M_j\leq{z})=\frac{1}{K}\sum_{k=1}^{K}\bigg(\prod\limits_{{i}=1}^{T^{(k)}_j}F_Y^{(d,j)}(z- X_{i}^{(j,k)})\bigg),\label{monmax_seasonality_overyears}
\end{equation} and the distribution of the annual maxima $M$ as\begin{equation}
    \mathbb{P}(M\leq z)=\frac{1}{K}\sum\limits_{k=1}^{K}\Bigg[\prod\limits_{j=1}^{12}\Bigg(\prod\limits_{{i}=1}^{T^{(k)}_j}F_Y^{(d,j)}(z- X_{i}^{(j,k)})\Bigg)\Bigg]\label{annmax_seasonality_allyr}.
\end{equation}

Note that $\mathbb{P}(M\leq z)\neq \prod_{j=1}^{12}\mathbb{P}(M^{(k)}\leq{z})$. The right hand side of this inequality does not impose a link in the tides to be from the same year across months.

==> RLs.tex <==
\textcolor{red}{(Thought - When plotting RL results, only plot return period 10 to 10000 rather than starting at 0.1 because some results were weird for low return periods??)} 

\textcolor{red}{Can I compare my RL ests with the outputs of CFB 2018 - have seen this done in another paper.}

%Alternatively, comparisons can be made with estimates obtained from fitting a model to annual maxima data (of sea levels); this is typically represented by a GEV. The model results were compared with those from the GEV model as a sense check. Then talk about largest deviations occurring at long return periods (higher or lower).Quality of fit varies by site? If our model overestimates with respect to the data; this represents less of an operational risk (than underestimate) but should be investigated further \citep{CFB2018}}

%\textcolor{red}{For ann max GEV - return levels are not compared at high return periods as the GEV model tends to underestimate these levels. For the empiricals - a visual comparison is made between the return levels estimated empirically from the data and the SSJPM return level curve. An assessment is made for low, med and high return periods for each gauge based on how well the curve fits to the data. \citep{CFB2018}}

%\textcolor{red}{Can also use CIs for model validation. In general, a low level of confidence is given to widths>1.5m, a medium to widths between 0.75 and 1.5m and a high level is assigned to widths <0.75m. The width of the interval is also balanced with the length of the data series therefore this assessment is perhaps prone to greater subjectivity \citep{CFB2018}}

For comparison purposes, we estimate return levels from the monthly and annual maxima distributions under four scenarios:
\begin{itemize}
    \item \textbf{Current method}: Seasonality is ignored in both skew surge and peak tide. The distribution of sea levels are given by equations \eqref{monmax_noseasonality} and \eqref{annmax_noseasonality} for the monthly and annual maxima respectively.
    \item \textbf{Proposed method}: We account for seasonality in both skew surge and peak tide using the distribution functions given in equations \eqref{monmax_seasonality_overyears} and \eqref{annmax_seasonality_allyr} for the monthly and annual maxima respectively.
    \item \textbf{Intermediate solution I}: We account for seasonality in skew surge but not in peak tides. So the monthly maxima distribution is given by equation \eqref{sldist_ss_stat}, using the seasonal skew surge model from equation \eqref{final_ss_model} but the tidal sample is taken from any temporal location. The annual maxima distribution is derived by assuming independence of the monthly maxima and taking the product over months.
    \item \textbf{Intermediate solution II}: We account for seasonality in peak tide but not in the skew surges. The distribution functions have the same form as those in the proposed method, but the skew surge model is replaced by the model in \eqref{ss_nonstat_model} where seasonality is ignored. We are still accounting for interannual tidal variations here.
\end{itemize}
We show the results for the current and proposed methods here, the results for both intermediate solutions are shown in Appendix \ref{extra_RLs}. 

For model validation, we compare our estimates with empirical estimates. This approach is restricted to return periods within the range of data, and is highly uncertain at longer return periods. This approach is not recommended as a valid method of estimating return levels, but is helpful to check whether the model is capturing the distributional properties of observed sea levels. Model fit is then determined by visual inspection %\textcolor{red}{Any other comparison/model validation we can do? Compare with fitting GEV to ann max sea levels.} 
We also use confidence intervals for model validation, however the width of an interval also depends on the length of the data series so this assessment is more subjective. \textcolor{red}{Still need to do CIs}

%Figures \ref{HEY_monmax_2} and \ref{LOW_monmax_2} show the return level estimates at Heysham and Lowestoft respectively, up to a return period of 10,000 years. We observe that the empirical estimates closely follows the curve representing the proposed method, this highlights the importance of accounting for seasonality in both components. Differences between estimates from the proposed and current methods across months are driven by the skew surge and tidal characteristics within that month. For example, in summer (May, June, July, August), when skew surges and tides are both low, ignoring their seasonality as in the current method yields a significant overestimate at both sites. Whereas in winter (November, December, January, February), the current method gives an underestimate because skew surges are most extreme. 

%There are also disparities between the two sites in Figures \ref{HEY_monmax_2} and \ref{LOW_monmax_2} for the same months, this is because the characteristics at the sites are also different. Since Lowestoft has a small tidal range, the difference between the proposed and current method estimates are mainly attributable to ignoring skew surge seasonality, as opposed to tidal seasonality. Figure \ref{LOW_monmax_4} demonstrates this. Whereas, some differences at Heysham are driven by skew surge seasonality as the skew surge range is comparable to that at Lowestoft, but Figure \ref{HEY_monmax_4} shows this is not always the case. Return level estimates for months close to the equinoxes (March, April, August, September, October) are higher when tidal seasonality is accounted for, regardless of whether skew surge seasonality is considered or not.

%\begin{figure}
%    \centering
%    \includegraphics[width=\textwidth]{HEY_monmax_3x4_2.pdf}
%    \caption{Monthly return level estimates at Heysham for the proposed method (cyan) and the current method (purple), compared with empirical estimates (red). We also show the highest astronomical tidal level (black dashed line).}
%    \label{HEY_monmax_2}
%\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{LOW_monmax_3x4_2.pdf}
    \caption{Monthly return level estimates at Lowestoft for the proposed method (cyan) and the current method (purple), compared with empirical estimates (red). We also show the highest astronomical tidal level (black dashed line).}
    \label{LOW_monmax_2}
\end{figure}

We also derive return level estimates from the annual maxima distribution in equation \eqref{annmax_seasonality_allyr}, the results at Heysham and Lowestoft are shown in Figure \ref{Annmax_2}. At both sites, the proposed method yields higher return level estimates beyond the 100 year return period. At the 10,000 year level, this is 10cm and 22cm higher than the current methodology at Heysham and Lowestoft respectively. This is a significant result in terms of coastal flood defence design; if return levels are underestimated, coastal defences may not be built high enough to withstand the most extreme sea levels. Our results agree with the findings of \cite{carter1981} who demonstrate the importance of accounting for within-year seasonal variations on return level estimates of wave heights. Their results show that assuming waves are identically distributed across a year resulted in an underestimate of return levels.

In Figure \ref{Annmax_2}, the empirical estimates at low and high levels are not captured by the return level curves. By considering the annual maxima distribution for each year individually, and deriving return level estimates for each year, we aim to understand if variations in the tides across years is driving these difference - if particular small or large annual maxima occurred in a year with particularly low or high tides.  We only estimate these for the proposed model, with distribution function given by equation \eqref{annmax_seasonality_givenyr}. Figure \ref{Annmaxbyyear} shows the results at Heysham and Lowesotft. It is clear to see that Heysham has a greater variation in return level estimates derived for each year specifically, since these changes are driven by tidal variation and Heysham has a large tidal range. Whereas this range is much smaller at Lowestoft since the tidal range is small. \textcolor{red}{Note: This is still ongoing work.}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{HEY_annmax_2.pdf}\includegraphics[width=0.5\textwidth]{LOW_annmax_2.pdf}
    \caption{Annual return level estimates at Heysham (left) and Lowestoft (right) for the proposed method (cyan) and the current method (purple), compared with empirical estimates (red). We also show the highest astronomical tidal level (black dashed line)}
    \label{Annmax_2}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{HEY_annmax_byyear1.pdf}\includegraphics[width=0.5\textwidth]{LOW_annmax_byyear.pdf}
    \caption{Annual return level estimates at Heysham (left) and Lowestoft (right) for the proposed method, derived from the annual maxima distribution for all years (cyan) and year specific annual maxima distributions (grey), compared with empirical estimates (red). We also show the highest astronomical tidal level (black dashed line).}
    \label{Annmaxbyyear}
\end{figure}   

\textcolor{red}{
Ideas for this Section
\begin{itemize}
    \item Does the quality of fit vary by site?
    \item Over or underestimation? What does this mean application wise? 
    \item In \cite{CFB2018} they assess model fit at low, medium and high return periods
    \item Confidence intervals.
\end{itemize}}


==> RLs2.tex <==
Using the distribution of the monthly and annual maxima sea levels derived in Section \ref{methodology}, we estimate return levels by solving \begin{equation}
    \mathbb{P}(M_j\leq z_p)=1-p \quad \text{and} \quad \mathbb{P}(M\leq z)=1-p
\end{equation} respectively for $p\in[0,1]$. We are interested in return levels up to the 10,000 year level, corresponding to annual exceedance probability $p=10^{-4}$. In the monthly case, this is the level we expect the monthly maxima $M_j$ to exceed every $1/p$ of that particular month (for example, every 100 Januarys), on average. Inverting the annual maxima distribution yields the level we expect the annual maxima to exceed every $1/p$ years on average.

We derive return level estimates from each stage in the modelling process outlined in Section~\ref{methodology}. We detail each of these below in a nested \textcolor{red}{best word?} list, so that each model builds on the previous method. Note that notation follows from Section~\ref{methodology},\begin{itemize}
    \item \textbf{Current method}: This is the methodology currently used in practice, where skew surges are assumed to be iid and peak tides are stationary. This is the same approach used in \cite{Tawn1992}, but they looked at storm surge and tides. The annual maxima distribution is given by \begin{equation}
        P(M\leq z)=\bigg(\prod\limits_{i=1}^{T} F(y-X_{i})\bigg)^{N/T}
    \end{equation} for $N$ the number of peak tides in a year, $T$ the total number of peak tides and $F(\cdot)$ the stationary skew surge distribution of equation~\eqref{ss_nonstat_model}. \textcolor{red}{Should I rewrite section 4.1 to have annual maxima with this form?}
    \item \textbf{Intermediate solution I}: This method is derived under the same assumptions as the current method, but we allow the number of tidal samples to vary with month and year, and recognise interannual variations in the tide by averaging over yearly tidal samples. The monthly and annual maxima distributions are given in equation~\eqref{aver_max}.
    \item \textbf{Intermediate solution II}: We account for within-year seasonality in skew surge but not in peak tides. So the monthly maxima distribution is given by equation \eqref{sldist_ss_stat}, using the seasonal skew surge model from equation \eqref{final_ss_model} but the tidal sample is taken from any temporal location. The annual maxima distribution is derived by assuming independence of the monthly maxima and taking the product over months.
    \item \textbf{Intermediate solution III}: Conversely to intermediate solution II, we account for seasonality in peak tide but not in the skew surges, so that the skew surge model of expression~\eqref{ss_nonstat_model} is used. The monthly and annual maxima distributions are given by the following, respectively, \begin{equation*}
        \mathbb{P}(M_j\leq{z})=\frac{1}{K}\sum\limits_{k=1}^{K}\prod\limits_{{i}=1}^{T_j^{(k)}}F_Y({z- X_{j_i}^{(k)}})\label{sldist_ss_stat}
        \mbox{ and }
        \mathbb{P}(M\leq{z})=\frac{1}{K}\sum\limits_{k=1}^{K}\prod\limits_{{j}=1}^{12}\prod\limits_{{i}=1}^{T_j^{(k)}}F_Y({z- X_{j_i}^{(k)}}).
    \end{equation*}
    \item \textbf{Proposed method I}: We account for within-year seasonality of both skew surge and peak tide, and interannual variations of peak tides, We derived this model in Section~\ref{acc_ss_seasonality} so that the monthly and annual maxima distributions are given in expression~\eqref{sldist_ss_stat}.
    \item \textbf{Proposed method II}: Non-stationarity is accounted for in both components and we also use the methodology outlined in Section~\ref{acc_ssmt_dep} to capture the skew surge dependence on peak tide, so that the skew surge distribution of expression~\eqref{ss_tidedep_model} is used. Therefore, the monthly and annual maxima distributions are given by the following, respectively, \begin{equation*}
        \mathbb{P}(M_j\leq{z})=\frac{1}{K}\sum\limits_{k=1}^{K}\prod\limits_{{i}=1}^{T_j^{(k)}}F_Y^{(d,j,x)}({z- X_{j_i}^{(k)}})\label{sldist_ss_stat}
        \mbox{ and }
        \mathbb{P}(M\leq{z})=\frac{1}{K}\sum\limits_{k=1}^{K}\prod\limits_{{j}=1}^{12}\prod\limits_{{i}=1}^{T_j^{(k)}}F_Y^{(d,j,x)}({z- X_{j_i}^{(k)}}).
    \end{equation*}
    \item \textbf{Proposed method III}: Non-stationarity and skew surge-peak tide are captured in this model, as well as temporal dependence in the skew surges. We used the methodology described in Section~\ref{ss_dep}, where the annual maxima distribution is given in expression~\eqref{eqn::sldist_exi}.
\end{itemize}

%We begin by deriving estimates when skew surge and peak tide seasonality is accounted for in Section~\ref{rl_sslty} from the distributions given in expressions~\eqref{monmax_seasonality_overyears} and \eqref{annmax_seasonality_allyr}. In Section~\ref{rl_tidedep} we derive estimates from our model that accounts for skew surge dependence on peak tide, described in Section~\ref{acc_ssmt_dep}. We then estimate return levels from our final model in Section~\ref{rl_tempdep}, where skew surge temporal dependence is also accounted for, as outlined in expressions~\eqref{eqn::sldist_exi_mon} and \eqref{eqn::sldist_exi}. Throughout this section, we compare our model estimates to those derived empirically, which we expect to be accurate for return periods less than the observation period. This approach is restricted to return periods within the range of data, and is highly uncertain at longer return periods, so this method provides no information about rarer events. We do not recommended this as a valid method of estimating return levels, but it is useful for checking whether the model is capturing the distributional properties of observed sea levels. Model fit is then determined by visual inspection. We present measures of uncertainty on our estimates in Section~\ref{rl_final} using bootstrapped confidence intervals; these are also useful for assessing model fit and comparing our estimates.

In Section~\ref{sl_seasonality} we use our model to find the probability an extreme sea level occurs in each month, given it is higher than some threshold, which we set at different return periods. This provides a nice visualisation that can be used for planning of coastal maintenance. 

\subsubsection{Accounting for Non-stationarity}\label{rl_sslty}
In this section we investigate the effect that accounting for non-stationarity of skew surge and peak tide has on sea level return level estimates. For comparison purposes, we estimate return levels from the monthly maximum distribution under four scenarios:
\begin{itemize}
    \item \textbf{Current method}: Within-year seasonality is ignored in both skew surge and peak tide. The distribution of sea levels are given by equations \eqref{monmax_noseasonality} and \eqref{annmax_noseasonality} for the monthly and annual maxima respectively.
    \item \textbf{Proposed method I}: We account for seasonality in both skew surge and peak tide using the distribution functions given in equations \eqref{monmax_seasonality_overyears} and \eqref{annmax_seasonality_allyr} for the monthly and annual maxima respectively.
    \item \textbf{Intermediate solution I}: We account for seasonality in skew surge but not in peak tides. So the monthly maxima distribution is given by equation \eqref{sldist_ss_stat}, using the seasonal skew surge model from equation \eqref{final_ss_model} but the tidal sample is taken from any temporal location. The annual maxima distribution is derived by assuming independence of the monthly maxima and taking the product over months.
    \item \textbf{Intermediate solution II}: We account for seasonality in peak tide but not in the skew surges. The distribution functions have the same form as those in the proposed method I, but the skew surge model is replaced by the model in \eqref{ss_nonstat_model} where seasonality is ignored. We are still accounting for interannual tidal variations here.
\end{itemize}
We are mainly interested in the differences between the return level estimates of the current method and proposed method I, but the intermediate solutions allow us to understand which components' seasonality is driving these differences. Note that in all scenarios, we account for interannual variations in peak tide by averaging over the monthly samples, as discussed in Section~\ref{acc_ss_seasonality}.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Updated_plots/Mon_1x4_MJSD_ssntlyLOW.pdf}
    \caption{Monthly return level estimates for Lowestoft in March, June, September and December, derived under the current method (purple), proposed method I (cyan) and intermediate solutions I (magenta) and II (blue).}
    \label{fig::monmax_ssntly_RL_LOW_1x4}
\end{figure}

Figure~\ref{fig::monmax_ssntly_RL_LOW_1x4} shows monthly return level estimates at Lowestoft, derived under these four scenarios. The most noticable feature is the difference between proposed method I and the current method in June, this reaches \textcolor{red}{1.5m} at the 10,000 year return level. Here, skew surges are particularly low, so ignoring their seasonality leads to major overestimation of return levels as demonstrated by the curve for the current method and intermediate solution II. This overestimation increases with return period. On the other hand, in December when skew surges are most extreme, ignoring seasonality results in underestimates of return levels. Since the tidal range at Lowestoft is narrow (see Section~\ref{data}), differences between proposed method I and intermediate solution II are small. However, at Heysham where the tidal range is wide, we observe great differences in March and September \textcolor{red}{more..}. At all sites and in all months, the empirical estimates lie closest to proposed method I, this highlights the importance of accounting for seasonality in both components.

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{Updated_plots/Ann_ssntlyLOW.pdf}
    \includegraphics[width=0.49\textwidth]{Updated_plots/Ann_ssntlyLOW_yrly.pdf}
    \caption{Annual return level estimates for Lowestoft, derived under proposed method I (cyan) and the current method (purple). The right plot shows return levels derived from the annual maxima distribution in each year, so that each grey curve corresponds to a yearly return level estimate.}
    \label{fig::Ann_ssnlty_RL_LOW}
\end{figure}

Figure~\ref{fig::Ann_ssnlty_RL_LOW} shows annual return level estimates derived from proposed method I and the current method at Lowestoft. The current method yields lower return level estimates for return periods greater than 3 years, with the difference between the curves increasing with return period. At the 10,000 year level, the current method gives a return level 23cm lower than proposed method I. It is difficult to make a comparison with the empirical estimate, since this is so variable, but the monthly return levels have already shown proposed method I lies closest to these (see Figure ~\ref{fig::monmax_ssntly_RL_LOW_1x4}). The right plot of Figure~\ref{fig::Ann_ssnlty_RL_LOW} shows return levels derived from the year specific annual maximum distribution of expression~\eqref{annmax_seasonality_givenyr} at Lowestoft. This tells us how much the return levels vary with tides year-to-year. Since Lowestoft has a small tidal range, these vary by no more than 30cm \textcolor{red}{check} at all return periods, whereas at Heysham...

\subsubsection{Accounting for Skew Surge Dependence on Peak Tide}\label{rl_tidedep}
In proposed method I, we account for seasonality in skew surge and peak tide, but we assume these components are independent. Here, we show the results from \textbf{proposed method II}, where seasonality is still accounted for but we also use the methodology outlined in Section~\ref{acc_ssmt_dep} to capture the skew surge dependence on peak tide. Return levels under proposed method II are derived from the monthly and annual maxima distributions given by expression~\eqref{monmax_seasonality_overyears} but with the skew surge distribution of equation~\eqref{ss_tidedep_model}. We compare our results with the empirical estimates and proposed method I, given in Section~\ref{rl_sslty}. We begin by presenting monthly maximum return levels because these reflect the non-stationarity of the dependence structure found in Section~\eqref{ss_mt_indep}. Then we give the annual maxima return levels to demonstrate the overall effect of ignoring skew-surge peak tide dependence. In this section, we focus on the results at Sheerness where the skew surge-peak tide dependence is strongest, as demonstrated in Section~\ref{ss_mt_indep}, but results for the remaining results are given in \cite{DarcySM}.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Updated_plots/Mon_1x4_MJSD_tidedepSHE.pdf}
    \caption{Monthly return level estimates for Sheerness in March, June, September and December, derived under proposed method I (cyan) and proposed method II (orange) where we account for and ignore skew surge-peak tide dependence, respectively.}
    \label{fig::Mon_tidedep_RL_SHE}
\end{figure}

Figure~\ref{fig::Mon_tidedep_RL_SHE} shows monthly return level estimates in March, June, September and December for proposed methods I and II, as well as those found empirically. Clearly, ignoring skew surge-peak tide dependence results in an overestimate of return levels, as expected. At the 10,000 year level, these are overestimated by 15.3, 13.7, 17.4 and 10.1cm in March, June, September and December, respectively. In Section~\ref{ss_mt_indep}, we concluded that it was reasonable to assume skew surge-peak tide independence in March, September and December, however our results demonstrate the consequences of this assumption. Proposed method II tends to lie closer to the empirical estimates, suggesting that accounting for this dependence is important and reflects the realism of the process.

Figure~\ref{fig::Ann_tidedep_RL} shows the annual return level estimates at Sheerness and Lowestoft, where we deemed it reasonable to assume skew surge and peak tide are independent in Section~\ref{ss_mt_indep}. The difference between proposed methods I and II is greater at Sheerness for all return levels, this reflects the stronger dependence observed at this site. Whereas at Lowestoft, accounting for this dependence when we know it is extremely weak, doesn't have an influence on return levels. Ignoring skew surge-peak tide dependence results in an overestimate of 13.8cm at the 10,000 year level at Sheerness, compared to an overestimate of 0.8cm at Lowestoft. Clearly, return level estimates from proposed method II lie closer to the empirical estimates at Sheerness, however, at Lowestoft the curves are indistinguishable at these shorter return periods. The significant results at Sheerness highlight the importance of accounting for this dependence, since overestimation of return levels can result in a waste of critical resources and over-expenditure.

\begin{figure}
    \centering
    \includegraphics[width=.49\textwidth]{Updated_plots/Ann_tidedepLOW.pdf}\includegraphics[width=.49\textwidth]{Updated_plots/Ann_tidedepSHE.pdf}
    \caption{Annual return level estimates for Lowestoft (left) and Sheerness (right) derived under proposed method I (cyan) and proposed method II (orange) where we account for and ignore skew surge-peak tide dependence, respectively.}
    \label{fig::Ann_tidedep_RL}
\end{figure}

\subsubsection{Accounting for Skew Surge Temporal Dependence}\label{rl_tempdep}
So far, we derived return levels under the assumption that skew surges are temporally independent. However, we know this isn't reasonable since storms tend to last multiple tidal cycles. In this section, we estimate return levels under \textbf{proposed method III} where we capture this temporal independence using the extremal index with a varying threshold level, as outlined in Section~\ref{ss_dep}. We focus on annual return levels derived under the model for the annual maximum given by expression~\eqref{eqn::sldist_exi}. As in previous sections, we compare these to empirical estimates, as well as proposed methods I and II.

Figure~\ref{fig::Ann_exiRL_LOW} shows the annual return level estimates derived under proposed methods I, II and III compared to the empirical estimates. The three proposed methods are almost indistinguishable at high return periods, greater than 100 years. However, for the lowest return periods, less than 10 years, proposed method III best matches the empirical estimates. This agrees with the known properties of the model given by expression~\eqref{eqn::exi_model} for temporal dependence, since the estimated extremal index is lower for lower skew surges, corresponding to lower return periods. But for the highest skew surges, and for any greater than those observed, $\hat\theta\rightarrow 1$, so the return level estimates remain unchanged for the rarest return periods. \textcolor{red}{Compare across sites, especially against HEY,}
\begin{figure}
    \centering
    \includegraphics[width=.49\textwidth]{Updated_plots/Ann_exiLOW.pdf}
    \caption{Annual return level estimates for Lowestoft derived under proposed method I (cyan), II (orange) and III (green). \textcolor{red}{Add in HEY when we have results}.}
    \label{fig::Ann_exiRL_LOW}
\end{figure}

\subsubsection{Final model}\label{rl_final}
\begin{itemize}
    \item Current, prop I II III all on one annual plot for each site
    \item Confidence intervals
    \item Comparison of fit across sites
    \item Assessment of fit?
\end{itemize}

==> Variations_in_loc.tex <==
The seasonal pattern is generally the same for a single component across Heysham, Lowestoft and Newlyn, in terms of the peaks and troughs observed in Figure \ref{ss_mt_bps_all}. However, the actual observed values of skew surge and peak tide vary significantly across sites. 

Table \ref{ranges} summaries the observed values at Heysham, Lowestoft and Newlyn. The peak tides observed at Heysham are higher than those at Newlyn, which are higher than those observed at Lowestoft. Additionally, than range of tides at Heysham is approximately fourfold than at Lowestoft. Whereas, the range of skew surges is greatest at Lowestoft and smallest at Heysham. The observed skew surges deviate less across sites than the peak tides, with the largest observations recorded at Lowestoft.

From Table \ref{ranges}, we see that Heysham is a tidally dominant site whilst Lowestoft is surge dominant. At Newlyn, the ranges are slightly more comparable but the tidal range is greater than that of the skew surges.

\begin{table}[]
    \centering
    \begin{tabular}{c||c|c|c||c|c|c||}
         & \multicolumn{3}{c||}{Skew surge (m)} & \multicolumn{3}{c||}{Peak tide (m)} \\ 
         & Range & Min & Max & Range & Min & Max \\
         Heysham & 2.794 & -1.107 & 1.688 & 4.263 & 6.418 & 10.681 \\
         Lowestoft & 3.392 & -1.469 & 1.923 & 1.006 & 1.935 &  2.941 \\
         Newlyn & 1.674 & -0.728 & 0.947 & 2.378 & 3.746 & 6.124
    \end{tabular}
    \caption{Range, minimum and maximum (meters) of skew surges and peak tides observed at Heysham, Lowestoft and Newlyn.}
    \label{ranges}
\end{table}

==> ex_ss_trends.tex <==
\textcolor{red}{Should I move this before we account for ss-pt dependence so that we get marginals correct first? Should it go before we account for temporal ss dependence or after?}

So far we have assumed that the only non-stationary features of extreme skew surges are in their mean value (addressed by removal of a linear trend in Section \ref{lineartrend}) and within year variations (described in Section \ref{acc_ss_seasonality}). In this section, we investigate if there are any longer-term trends in the extreme skew surges that we should incorporate into our model. We can capture these trends through the parameters of the GPD model for extreme skew surges. We do not consider modelling the shape parameter as we have fixed this across months, and this parameter is associated with the most uncertainty. We adapt the parameterisations of $\sigma$ and $\lambda$ in our model to account for longer-term trends and check for any improvement in model fit. 

Here, we adapt the skew surge model of Section \ref{acc_ss_seasonality}, with scale parameter defined by expression \eqref{sinescale}. We introduce a linear trend for each season using an indicator function, so that the scale parameter is given by \begin{equation}
        \sigma_{(d, k_n)} =a+b\sin\bigg(\frac{2\pi}{365}(d-\phi)\bigg)+\sum\limits_{s=1}^{4}\gamma_s k_n \mathbb{I}_{\{d\in S_s\}}\label{scale_lineartrend}
\end{equation} where $S_s$ for $s=1,\ldots,4$ indicates the seasons Winter, Spring, Summer and Autumn respectively. Then each season has it's own linear trend given by $\gamma_s k_n$ where $k_n\in[-1,1]$ denotes the year on a normalised scale common across sites and $\gamma_s$ the trend parameter. %We define the time variable by \begin{equation*}
    %t_n = \frac{t- t_{\text{med}}}{t_{\text{range}}/2}
%\end{equation*} where $t$ is the year of observation, $t_{\text{med}}$ the median year of the study period and $t_{\text{range}}$ the range of years of the study period. To allow comparison across sites, we use a common $t_n$, so that the median and range of Newlyn are used since this has the greatest study period. So  $t_{\text{med}} $ and $t_{\text{range}}$ are fixed across sites at 1964 and 49 respectively.

We fit the skew surge model with the updated scale parameter at each site using likelihood techniques. The estimates of $a,b,\phi$ and $\xi$ do not change significantly from those given in Table \ref{ss_param_ests}. Table \ref{paramests_lm} gives the linear trend parameter estimates $\hat\gamma_s$. The results across sites vary, based on AIC and BIC scores reported in Table \ref{AICBIC_lm}. Since the 95\% confidence intervals of some parameter estimates contain zero, we also considered cases where we set $\gamma_s=0$ for some $s$, so that not every season has a linear trend. We omit the details. 

\begin{table}[]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|c|c|c|c}
         & Heysham & Lowestoft & Newlyn & All\\ \hline
         $\hat\gamma_1$ & 0.031 (-0.022, 0.084)  & -0.0048 ( -0.058, 0.048) & 0.0049 (-0.009, 0.018) & 0.007 (-0.005, 0.019) \\
         $\hat\gamma_2$ & 0.031 (-0.0054, 0.068) & -0.0136 (-0.044, 0.017)  & 0.011 (0.002,0.019) & 0.010 (0.002, 0.018) \\
         $\hat\gamma_3$ & -0.029 (-0.053, -0.0043) & 0.018 (-0.0051, 0.042) & -0.002 (-0.005, 0.004) & -0.002 (-0.007, 0.004) \\
         $\hat\gamma_4$ & -0.026 (-0.069,0.016) & 0.012 (-0.029, 0.052) & 0.0089 (0.001, 0.018) & 0.0075 (-0.001, 0.016) \\
    \end{tabular}
    }
    \caption{Estimates of the seasonal linear trend parameters when fitting the skew surge model of equation $\eqref{final_ss_model}$ with scale parameter in equation $\eqref{scale_lineartrend}$ at Heysham, Lowestoft and Newlyn. The final column shows seasonal linear trend parameter estimates when fitting the same model but with the scale parameter in equation \eqref{scale_lineartrend_allsites}, so that the trend is the same at all sites. 95\% confidence intervals are given in parentheses.}
    \label{paramests_lm}
\end{table}

Notice in Table \ref{paramests_lm}, there is considerable overlap between $\hat\gamma_s$ for each $s$ across sites. Therefore, we investigate fitting a common seasonal linear trend parameter across sites. We add another covariate on the scale parameter to indicate the site $L=1,2,3$ corresponding to Heysham, Lowestoft and Newlyn respectively. We still use a separate harmonic at each site because the seasonality of the skew surges are not identical. The scale parameter is now given by \begin{equation}
    \sigma_{(d,k_n,L)} =\sum\limits_{l=1}^{3}\bigg[a_l+b_l\sin\bigg(\frac{2\pi}{365}(d-\phi_l)\bigg)\bigg]\mathbb{I}_{\{L=l\}}+\sum\limits_{s=1}^{4}\gamma_s k_n \mathbb{I}_{\{d\in S_s\}}.\label{scale_lineartrend_allsites}
\end{equation}
A common shape parameter for the GPD is used across sites, this is justified by the overlap of the confidence intervals for the separate site analysis (see Table \ref{ss_param_ests}). Comparing AIC and BIC in Table \ref{AICBIC_lm}, we do not observe an improvement on model fit when this linear trend is incorporated, although the AIC scores are close.

\begin{table}[]
    \centering
    %\resizebox{\textwidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
         & \multicolumn{2}{c|}{Heysham} & \multicolumn{2}{c|}{Lowestoft} & \multicolumn{2}{c|}{Newlyn} & \multicolumn{3}{c}{All} \\
         & None & All & None & All & None & All & None & All & Final  \\ \hline
         AIC & 0 & -4.17 & 0 & 3.50 & 0 & -2.69 & 0 &  1.06 & -4.39 \\
         BIC & 0 & -64.15 & 0 & 25.23 & 0 & 21.20 & 0 &  24.87 & -0.69 \\
    \end{tabular}
    %}
    \caption{AIC and BIC scores for the fit of the skew surge model of equation $\eqref{final_ss_model}$ with scale parameter in equation $\eqref{sinescale}$ with a linear trend for each season (All) relative to no linear trend in $\eqref{scale_lineartrend}$ (None) at Heysham, Lowestoft and Newlyn. The final column shows the scores when fitting the same model but with a linear trend common to all sites for each season (All) and a common linear trend for autumn, winter and spring, but no trend in Summer (Final).}
    \label{AICBIC_lm}
\end{table}

We then investigate pooling various combinations of seasons together whilst setting other seasons to zero; this is motivated by the confidence intervals of parameter estimates overlapping or containing zero. AIC and BIC scores both suggest that the best model fit is one with a common linear trend across sites and across autumn, winter and spring; so that the summer linear trend parameter is set to zero \textcolor{red}{Differences in AIC/BIC are small though}. For this model, the scale parameter is defined by 
\begin{equation}
    \sigma_{(d,k_n,L)} =\sum\limits_{l=1}^{3}\bigg[a_l+b_l\sin\bigg(\frac{2\pi}{365}(d-\phi_l)\bigg)\bigg]\mathbb{I}_{\{L=l\}}+\gamma_s k_n \mathbb{I}_{\{d\in S_1,S_2,S_4\}}.\label{scale_lineartrend_final}
\end{equation}
So that if the day observation $d$ lies in seasons $S_1,S_2$ or $S_4$ (winter, spring or autumn), then the linear trend parameter $\gamma_s$ is used; otherwise if the day lies in summer, there is no seasonal trend parameter. Using likelihood inference we estimate this parameter as $\hat\gamma_s=0.00838$ (95\% confidence intervals is [0.00299, 0.0138]), this corresponds to an annual increase of 0.171mm in extreme skew surges.

==> impact_seasonality.tex <==
\textcolor{red}{Not sure how much of the derivation to give here or whether to move to supplementary material.}

Using our model, we explore the seasonality of sea levels. We are interested in the following probability: \begin{equation}
    p_j=\mathbb{P}(M\in j\; |\;M=z).\label{p_eq}
\end{equation} for months $j=1,\ldots,12$, $M$ the annual maxima of sea levels, and $z\in\mathbb{R}$. We evaluate this empirically, and also using our model to extrapolate $z$ beyond the range of observed data. Increasing $z$ to rare return levels uncovers the seasonal variations in the sea level distribution. For months where the most extreme sea levels are observed, $p_j$ take it's largest values, whilst $p_j\rightarrow 0$ for months where the least extreme sea levels are observed. In this section, we derive the form of $p_j$ when using our model. The results are shown in Section \ref{sl_seasonality}.


First, we condition on a fixed year $k$ and consider the probability $p_j^{(k)}$. We can rewrite this in terms of the distribution and density of the monthly maxima sea level, $F_{M_j^{(k)}}$ and $f_{M_j^{(k)}}$ respectively, and the density of the annual maxima sea level $f_{M^{(k)}}$, each conditional on some year $k$: \begin{equation}
    p_j^{(k)}=\frac{1}{f_{M^{(k)}}(z)}\bigg[\bigg(\frac{f_{M_{j}^{(k)}}(z)}{F_{M_j^{(k)}}(z)}\bigg)F_{M^{(k)}}(z)\bigg].
\end{equation}
It follows to find an expression for each of these terms to simplify the above equation.

To find the form of the density of the monthly maxima sea levels, this requires differentiation via the product rule of the skew surge distribution function (see equation \eqref{final_ss_model}). So we must first formulate the density of the skew surges $f_{Y}^{(d,j)}$. Below the threshold, where the monthly empirical distribution is used, we estimate the monthly empirical density using a Gaussian kernel density estimate. Denote this $\hat f_j$. Above the threshold, we differentiate to yield the density function. This gives \begin{align}
    f_{Y}^{(d,j)}(z-X_{j_i}^{(k)})=\begin{cases}  \hat f_j(z-X_{j_i}^{(k)}) \quad\quad &\text{if } z-X_{j_i}^{(k)}\leq u_j \\ \\ \frac{\lambda_d}{\sigma_d}\big[1+\xi\big(\frac{(z-X_{j_i}^{(k)})-u_j}{\sigma_d}\big)\big]^{-\frac{1}{\xi}-1} \quad &\text{if }z-X_{j_i}^{(k)}> u_j. \label{ss_den_abu}
    \end{cases}
\end{align} Then we can write the density of the monthly maxima sea levels as \begin{align}
    f_{M_j^{(k)}}(z) &= \prod\limits_{i=1}^{T_{j}^{(k)}}F_{Y}^{(d,j)} (z-X_{j_i}^{(k)})\sum\limits_{i=1}^{T_{j}^{(k)}}\frac{{f_Y}^{(d,j)}(z-X_{j_i}^{(k)})}{F_{Y}^{(d,j)}(z-X_{j_i}^{(k)})}\\
    &= F_{M_{j}^{(k)}}(z-X_{j_i}^{(k)})\sum\limits_{i=1}^{T_{j}^{(k)}}\frac{{f_Y}^{(d,j)}(z-X_{j_i}^{(k)})}{F_{Y}^{(d,j)}(z-X_{j_i}^{(k)})}\label{monmax_sldensity}
\end{align} where the density of the skew surges $f_{Y}^{(d,j)}$ is given above.

To find the density of the annual maxima of sea levels, we follow the same approach by differentiating the form of the annual maximum distribution function for a given year.
\begin{align}
    f_{M^{(k)}}(z)&=\prod\limits_{j=1}^{12}\prod\limits_{i=1}^{T^{(k)}_j}F_{Y}^{(d,j)}({z-X_{j_i}^{(k)}})\sum\limits_{j=1}^{12}\sum\limits_{j_i=1}^{T_{j,k}}\frac{f_Y^{(d,j)}(z-X_{j_i}^{(k)})}{F_{S}^{(d,j)}({z-X_{j_i}^{(k)}})} \\ &= F_{M^{(k)}}(z)\sum\limits_{j=1}^{12}\sum\limits_{i=1}^{T_{j,k}}\frac{f_Y^{(d,j)}(z-X_{j_i}^{(k)})}{F_{Y}^{(d,j)}({z-X_{j_i}^{(k)}})}\label{annmax_sldensity}.
\end{align}
Then using equations \eqref{monmax_sldensity} and \eqref{annmax_sldensity}, we can rewrite $p_j{(k)}$ as \begin{equation}
    {p}_j^{(k)}
    = \frac{\sum\limits_{i=1}^{T_{j}^{(k)}}\frac{f_Y^{(d,j)}(z-X_{j_i}^{(k)})}{F_{Y}^{(d,j)}({z-X_{j_i}^{(k)}})}}{\sum\limits_{j=1}^{12}\sum\limits_{i=1}^{T_{j}^{(k)}}\frac{f_Y^{(d,j)}(z-X_{j_i}^{(k)})}{F_{Y}^{(d,j)}({z-X_{j_i}^{(k)}})}},
\end{equation} which we can see clearly sums to 1 over all months $j=1,\ldots,12$. Then, considering the probability over all years we get \begin{equation}
     {p}_j= \frac{1}{K}\sum\limits_{k=1}^{12} \frac{\sum\limits_{i=1}^{T_{j}^{(k)}}\frac{f_Y^{(d,j)}(z-X_{j_i}^{(k)})}{F_{Y}^{(d,j)}({z-X_{j_i}^{(k)}})}}{\sum\limits_{j=1}^{12}\sum\limits_{i=1}^{T_{j}^{(k)}}\frac{f_Y^{(d,j)}(z-X_{j_i}^{(k)})}{F_{Y}^{(d,j)}({z-X_{j_i}^{(k)}})}}.
\end{equation}

==> interann_variation.tex <==
\textcolor{red}{Briefly explain why tides vary and why important to account for variations - maybe add into background section - nodal and perigean cycles}

Since we are accounting for interannual tidal variations, we begin by deriving the distribution of the monthly maxima for a fixed year. We edit our notation so that we know the year, as well as the month, of observation. We denote the year by $k=1,\ldots,K$ for $K$ total years of observation. We now write the sequence of sea level random variables in month as \begin{equation}
    \{Z_{i_{(j,k)}}^{(j,k)}: i_{(j,k)}=1,\ldots,T_{j}^{k}, \;j=1,\ldots,12, \;k=1,\ldots,K\}
\end{equation} where $i_{(j,k)}$ represents the tidal cycle index in month $j$ and year $k$. Note that the number of tidal cycles changes monthly and annually, depending of the number of days in a month and the timing of the first cycle.  So we are interested in \begin{equation}
    \mathbb{P}(M_j^{(k)}\leq{z})=\mathbb{P}(\max\{Z^{(j,k)}_{i_{(j,k)}}:i_{(j,k)}=1,\ldots,T_{j}^{(k)}\}\leq{z}).
\end{equation}
%We rewrite this in terms of the skew surge and maximum tidal components, also accounting for their temporal location. In the proceeding sections, we challenge the stationarity assumption of these components, so their temporal location is important. To account for tidal variations across years, we condition on the tidal regime from the year of interest $k$. Assuming skew surges are independent, we obtain

We rewrite this in terms of the skew surge and peak tide components, adopting the same notation for the tidal regime: $X_{i_{(j,k)}}^{(j,k)}$. To account for tidal variations across years, we condition on the tidal regime from the year as well as the month of interest. Assuming skew surges are independent and incorporating the seasonal model from \eqref{final_ss_model}, we obtain

\begin{equation}
    \mathbb{P}(M_j^{(k)}\leq{z})=\prod\limits_{{i_{(j,k)}}=1}^{T^{(k)}_j}\mathbb{P}(Y_{i_{(j,k)}}^{(j)}\leq{z- X_{i_{(j,k)}}^{(j,k)}}| X_1^{(j,k)},\ldots,\tilde X_{T_{j}^{(k)}}^{(j,k)})=\prod\limits_{{i_{(j,k)}}=1}^{T^{(k)}_j}F(z- X_{i_{(j,k)}}^{(j,k)}).
\end{equation}

To derive the distribution of the monthly maxima across all years, we assume that each annual tidal regime has an equal probability of occurrence, so we can simply average over all of the possible regimes, so that
\begin{equation}
    \mathbb{P}(M_j\leq{z})=\frac{1}{K}\sum_{k=1}^{K}\bigg(\prod\limits_{{i_{(j,k)}}=1}^{T^{(k)}_j}F(z- X_{i_{(j,k)}}^{(j,k)})\bigg).\label{monmax_noseasonality_overyears}
\end{equation}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> method_simple.tex <==
For skew surges, it is important to model all observations. We are particularly interested in modelling extreme values to allow extrapolation to rare return levels. Extreme skew surges are defined as threshold exceedances, so we use the GPD formulation given in Section~\ref{evmethods} for modelling. Since extreme sea levels can occur with moderate skew surges at the largest peak tides we must also model values below the threshold; the empirical distribution of skew surge is suitable here. Therefore a model for the skew surges under an iid assumption is given by, \begin{align}
    F_{Y}(y)=\begin{cases} \tilde{F}_Y(y) \quad\quad &\text{if }y\leq u\\ \\ 1-\lambda_u\big[1+\xi\big(\frac{y-u}{\sigma_u}\big)\big]^{-1/\xi}  &\text{if }y> u \end{cases}\label{ss_nonstat_model}
\end{align} where $u$ is a high threshold, $\tilde F_Y$ the empirical distribution, $\lambda_u=1-\tilde{F}_Y(u)$ and $\sigma_u,\xi$ parameters of the GPD as in equation~\eqref{GPD_form}. 

Assuming that skew surge is independent of peak tide, we have that for all $i$ \begin{equation}
    \mathbb{P}(Z_i\leq z)=\mathbb{P}(Y_i\leq z-X_i)=F_{Y}(z-X_i),
\end{equation}
for $-\infty<z<\infty$. To overcome sampling variation of the tides, we average over a number of tidal cycle samples $S$ and denote each sample $s$ for $s=1,\ldots,S$. Assuming all months have an equal number of tidal cycles $T$, we write the distribution of $M_j$ as
\begin{equation}
    \mathbb{P}(M_j\leq z)=\frac{1}{S}\sum\limits_{s=1}^{S}\bigg(\prod\limits_{i=1}^{T}\mathbb{P}(Y_i\leq z- X_{i}^{(s)})\bigg)
    =\frac{1}{S}\sum\limits_{s=1}^{S}\bigg(\prod\limits_{i=1}^{T}F_{Y}(z- X_{i}^{(s)})\bigg),\label{monmax_noseasonality}
\end{equation}
where $\{X_i^{(s)}\}_{i=1}^{T}$ is a sequence of consecutive peak tides. Since peak tides are not temporally independent of each other, the sample must be contiguous but this sequence can start anywhere in the time series, under the assumption of peak tide stationarity. The annual maxima distribution is given by,
\begin{equation}
    \mathbb{P}(M\leq z)  =\prod\limits_{j=1}^{12}\bigg[\frac{1}{S}\sum\limits_{s=1}^{S}\bigg(\prod\limits_{i=1}^{T}F_{Y}(z- X_{i}^{(s)})\bigg)\bigg].\label{annmax_noseasonality}
\end{equation} We fit this model to our data, with $\lambda_u=0.05$, and derive return level estimates in Section \ref{results}.

%From these distributions, we can estimate monthly and annual return levels. Solving \begin{equation}
 %   \mathbb{P}(M_j\leq z_p)=1-p \quad \text{for } p\in(0,1),
%\end{equation} gives us the monthly return level $z_p$ associated with return period $1/p$. This is the level we expect the monthly maxima of the sea levels $M_j$ to exceed every $1/p$ years (in month $j$), on average. To find the levels expected to be exceeded by the annual maxima, we solve 
%\begin{equation}
%    \mathbb{P}(M\leq z_p)=1-p \quad \text{for } p\in(0,1).
%\end{equation} Note that $p$ denotes the annual exceedance probability, so for rare events we are particularly interested in $p=10^{-4}$ which corresponds to a return period of 10,000 years. Here, we are extrapolating far beyond what has been observed so these estimates are subject to much uncertainty.

==> sealevelcomponents.tex <==
\cite{pughwoodworth2014} give a comprehensive overview of the sea level processes, we discuss the relevant ideas here. Sea levels are primarily determined by the tidal regime. Tides are the predictable rise and fall of the sea surface that result from the gravitational interaction between the Earth, Moon and Sun. This astronomical process is deterministic and well understood, so that tides can be predicted many years into the future with a high degree of accuracy (see \cite{egbert2017} for details on tidal prediction). 

In the UK, the tidal regime is semi-diurnal because a full tidal cycle of one high tide and one low tide takes approximately 12 hours 25 minutes. The timing and magnitude of low and high tides varies across the UK coastline. The range of semi-diurnal tides typically follow a 14 day cycle, where the greatest ranges are observed when the Sun and Moon are in line with the Earth at full or new Moon, this is known as spring tide. Periods of smaller tidal ranges are called neap tides, when the sun and moon are perpendicular to the Earth. Interannual variations in tides result from modulations in the semi-diurnal tidal ranges. Longer-term tidal cycles are also driven by astronomically, including the 18.6 year lunar nodal cycle and the 8.85 year cycle of lunar perigee.


Storm surges are short-term sea level changes resulting from the weather. They are caused by low atmospheric pressure and strong winds forcing high waters towards the coastline. Storm surges can only be forecast with the same time horizon as the weather. Due to the complex dependence structure between tide and storm surge, we focus on skew surge as an alternative measure of the meteorological forcing on sea levels (see Figure \ref{ssexplan}). \cite{Williams2016} demonstrate that is it reasonable to assume skew surge and peak tide are independent.

==> suppfig.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SUPP FIGS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section{Supplementary Figures}

%\subsection{Skew Surge and Peak Tide Seasonality}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.49\textwidth]{Updated_plots/ss_bp_LOW.pdf}    \includegraphics[width=0.49\textwidth]{Updated_plots/mt_bp_LOW.pdf}    \includegraphics[width=0.49\textwidth]{Updated_plots/ss_bp_NEW.pdf}    \includegraphics[width=0.49\textwidth]{Updated_plots/mt_bp_NEW.pdf}
    \includegraphics[width=0.49\textwidth]{Updated_plots/ss_bp_SHE.pdf}    \includegraphics[width=0.49\textwidth]{Updated_plots/mt_bp_SHE.pdf}
    \caption{Skew surge (left) and peak tide (right) monthly boxplots at Lowestoft (top), Newlyn (middle) and Sheerness (bottom)}
    \label{ss_mt_bps_all}
\end{figure}

%In Section \ref{ss_seasonality}, we discussed the within-year seasonality of skew surge and peak tide. At Heysham (Figure \ref{ss_mt_bps_HEY}), peak tides are greatest in March and September. Figure \ref{ss_mt_bps_all} shows the a boxplot per month for the distribution of skew surge and peak tide at Lowestoft, Newlyn, and Sheerness. We observe the same seasonality for all sites. At Newlyn the autumn peak is slightly greater than the spring peak. The median of the peak tides is fairly constant across months for Heysham, Newlyn and Sheerness. However, at Lowestoft the median has a clear seasonal pattern, reaching its lowest point in March before steadily increasing to its peak in October. The upper tail of the distributions still peak in spring and autumn, but the autumn peak is significantly larger.

%Figure \ref{mt_seasonality_plot} shows the estimates of $p_j(q;R)$ defined in equation \eqref{prob}, for $R$ representing peak tides and for various quantiles $q$ at Lowestoft, Newlyn and Sheerness. We also add 95\% confidence intervals to the estimates of $p_j(0.999;R)$ at each site. A full discussion of these results is given in Section \ref{ss_seasonality}. 

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{Updated_plots/maxtide_LOW.pdf}
    \includegraphics[width=0.49\textwidth]{Updated_plots/maxtide_CI_LOW.pdf}
    \includegraphics[width=0.49\textwidth]{Updated_plots/maxtide_NEW.pdf}
    \includegraphics[width=0.49\textwidth]{Updated_plots/maxtide_CI_NEW.pdf}
    \includegraphics[width=0.49\textwidth]{Updated_plots/maxtide_SHE.pdf}
    \includegraphics[width=0.49\textwidth]{Updated_plots/maxtide_CI_SHE.pdf}
    \caption{Estimates of $\hat p_j(R;q)$ (see expression~\eqref{prob}) for months $j=1,\ldots,12$ at $q=0.5$ (black), 0.9 (pink), 0.95 (magenta), 0.99 (purple) and 0.999 (blue) for Lowestoft (top), Newlyn (middle) and Sheerness (bottom) in the left column. We also show the 95\% confidence intervals for $\hat p_j(R;0.999)$ estimates at each site (right column).}
    \label{mt_seasonality_plot}
\end{figure}

%\subsection{Skew Surge and Peak Tide Dependence}
%Figure \ref{ss_mt_scatter} shows extreme skew surge (defined as exceedances of the 0.95 quantile) against their associated ranked peak tide (over all peak tides) at each site. The tides are ranked so that 1 corresponds to the smallest peak tide observation. If the two components are independent, ranked peak tides associated with extreme skew surges will be uniformly distributed. We test this formally using a Kolmogorov-Smirnov test for uniformity~\citep{kolmogorov1933} and discuss the results in Section \ref{ss_mt_indep} and Section \ref{ss_mt_indep_supp}.

\begin{table}[]
    \centering\resizebox{\textwidth}{!}{
    \begin{tabular}{c|c||c|c|c|c}
         & Block size & 0.9 & 0.95 & 0.975 & 0.99\\ \hline
        %HEY & 10 & 0.00288 & 0.0336 & 0.1313 & 0.095 \\
        HEY & 19 &  & 0.044 (0.082) &  &   \\
        LOW & 5 & 0.63 (0.17) & 0.72 (0.22) & 0.78 (0.27) & 0.33 (0.23) \\
        NEW & 20 & 0.070 (0.075) & 0.091 (0.087) & 0.15 (0.17) & 0.12 (0.11)  \\
        SHE & 6 & 1.5$\times 10^{-8}$ (4.1$\times{10^{-8}}$) & 1.1$\times 10^{-4}$ (2.9 $\times 10^{-4}$) & 9.9 $\times{10^-4}$ (-0.0011) & 0.0013 (7.0$\times{10^{-4}}$) \\
    \end{tabular}
    }
    \caption{K-S test $p$ values uniformity of ranked peak tides associated with extreme skew surges, defined as exceedances of different quantiles of the data. Average $p$ values after repeated bootstrapping are shown in parentheses.}
    %%%%% Needs updating for NEW
    \label{KStest_threshold}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{Updated_plots/exss_mt_scatter_HEY.pdf}
    \includegraphics[width=0.48\textwidth]{Updated_plots/exss_mt_scatter_LOW.pdf}\\
    \includegraphics[width=0.48\textwidth]{Updated_plots/exss_mt_scatter_NEW.pdf}
    \includegraphics[width=0.48\textwidth]{Updated_plots/exss_mt_scatter_SHE.pdf}
    \caption{Extreme skew surge observations against associated rank peak tides at Heysham (top right), Lowestoft (top left), Newlyn (bottom left) and Sheerness (bottom right)}
    \label{ss_mt_scatter}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{pdf_mt_HEY.pdf}\includegraphics[width=0.4\textwidth]{Updated_plots/mt_pdf_LOW.pdf}\\
    \includegraphics[width=0.4\textwidth]{Updated_plots/mt_pdf_NEW.pdf}\includegraphics[width=0.4\textwidth]{Updated_plots/mt_pdf_SHE.pdf}
    \caption{Distribution of peak tides at Heysham (top left), Lowestoft (top right), Newlyn (bottom left) and Sheerness (bottom right). Probability density function of all peak tides (black) and probability density function peak tides associated with extreme skew surges (red) are interpolated onto each distribution.}
    \label{pdf_mt}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Updated_plots/mt_quantreg_HEY.pdf}\includegraphics[width=0.45\textwidth]{Updated_plots/mt_quantreg_LOW.pdf}\\
    \includegraphics[width=0.45\textwidth]{Updated_plots/mt_quantreg_NEW.pdf}\includegraphics[width=0.45\textwidth]{Updated_plots/mt_quantreg_SHE.pdf}
    \caption{0.95 quantile estimates of skew surges associated with groups of ordered peak tides of size 100, at Heysham (top left), Lowestoft (top right), Newlyn (bottom left) and Sheerness (bottom right).}
    \label{quantile_reg}
\end{figure}

%\subsection{Parameter Estimates for Extreme Skew Surges}
%Figure \ref{ss_param_ests_fig_all} shows the GPD model parameter estimates for Lowestoft, Newlyn and Sheerness for the monthly model discussed in Section \ref{acc_ss_seasonality} and Model $B$, with scale parameter defined by equation \ref{sinescale}. Each site shows the same pattern in scale parameter as Heysham, in Figure \ref{ss_param_ests_fig_HEY}, where values are higher in Winter than Summer. Whereas, the monthly model shape parameter estimates remain relatively constant across months, except for May at Lowestoft. However, fixing the shape parameter across still yields the best model fit (see Table \ref{AICBIC_ss}). Notice that the 95\% confidence intervals on parameter estimates are much narrower at Newlyn due to the amount of data available. 


\begin{figure}[h]
    \entering
    \includegraphics[width=0.5\textwidth]{Updated_plots/scale_paramest_LOW.pdf}\includegraphics[width=0.5\textwidth]{Updated_plots/shape_paramest_LOW.pdf}
    \includegraphics[width=0.5\textwidth]{Updated_plots/scale_paramest_NEW.pdf}\includegraphics[width=0.5\textwidth]{Updated_plots/shape_paramest_NEW.pdf}
    \includegraphics[width=0.5\textwidth]{Updated_plots/scale_paramest_SHE.pdf}\includegraphics[width=0.5\textwidth]{Updated_plots/shape_paramest_SHE.pdf}
    \caption{Scale (left) and shape (right) parameter estimates for Model $S2$ (blue) and the monthly model (black) at Lowestoft (top), Newlyn (middle) and Sheerness (bottom).}
    \label{ss_param_ests_fig_all}
\end{figure}

%\subsection{Accounting for Skew Surge Temporal Dependence}
%Figure \ref{fig::acf_ss} shows the autocorrelation function (acf) plot for each site. These aid with choosing a block size for the non-stationary bootstrap procedure in Section \ref{ss_mt_indep} and Section \ref{ss_mt_indep_supp}, and with run length for the runs estimate in Section \ref{ss_dep}. Figure \ref{fig::exi_vartrl} shows estimates of the extremal index using the runs estimate, for various run lengths and threshold at each location. Figures \ref{fig::chi} and \ref{fig::chibar} show plots of the extremal dependence measures $\chi$ and $\bar\chi$ (see Section \ref{sec::suppmat_exi}) for various high quantiles and for each site. %The extremal index is higher for higher thresholds, as expected since exceedances of higher thresholds are less likely to be dependent and cluster. As run length increases, the extremal index decreases 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{Updated_plots/acf_skews_HEY.pdf}\includegraphics[width=0.45\textwidth]{Updated_plots/acf_skews_LOW.pdf} \\
    \includegraphics[width=0.45\textwidth]{Updated_plots/acf_skews_NEW.pdf}\includegraphics[width=0.45\textwidth]{Updated_plots/acf_skews_SHE.pdf}
    \caption{Autocorrelation function plots for Heysham (top right), Lowestoft (top left), Newlyn (bottom right) and Sheerness (bottom left).}
    \label{fig::acf_ss}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{Updated_plots/EI_runs_HEY.pdf}    \includegraphics[width=0.45\textwidth]{Updated_plots/EI_runs_LOW.pdf}\\
    \includegraphics[width=0.45\textwidth]{Updated_plots/EI_runs_NEW.pdf}
    \includegraphics[width=0.45\textwidth]{Updated_plots/EI_runs_SHE.pdf}
    \caption{Runs estimate of the extremal index for skew surge, at various quantiles and run lengths. The quantiles are 0.9 (black), 0.95 (red), 0.975 (blue), 0.99 (green) and 0.999 (orange).}
    \label{fig::exi_vartrl}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.85\textwidth,height=5cm]{Updated_plots/chi_HEY.pdf} \\
    \includegraphics[width=0.85\textwidth,height=5cm]{Updated_plots/chi_LOW.pdf} \\
    \includegraphics[width=0.85\textwidth,height=5cm]{Updated_plots/chi_NEW.pdf} \\
    \includegraphics[width=0.85\textwidth,height=5cm]{Updated_plots/chi_SHE.pdf}
    \caption{$\chi$ for Heysham, Lowestoft, Newlyn and Sheerness (from top to bottom) for exceedances of the 0.9, 0.95, 0.975, 0.99 and 0.999 quantiles for various lags.}
    \label{fig::chi}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{Updated_plots/EI_model_LOW.pdf}
    \includegraphics[width=0.49\textwidth]{Updated_plots/EI_model_NEW.pdf}
    \includegraphics[width=0.49\textwidth]{Updated_plots/EI_model_SHE.pdf}
    \caption{Estimates of the subasymptotic extremal index $\theta(y,r)$ for different skew surge levels using the runs estimate (black) and our model estimate (red) of expression~\eqref{eqn::exi_model} at Lowestoft (top left), Newlyn (middle) and Sheerness (bottom). Run lengths are chosen as 10, 2 and 10, respectively. And the threshold $v$ is chosen as the 0.99 skew surge quantile at all sites.}
    \label{fig::exifun_all}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.85\textwidth,height=5cm]{Updated_plots/chibar_HEY.pdf} \\
    \includegraphics[width=0.85\textwidth,height=5cm]{Updated_plots/chibar_LOW.pdf} \\
    \includegraphics[width=0.85\textwidth,height=5cm]{Updated_plots/chibar_NEW.pdf} \\
    \includegraphics[width=0.85\textwidth,height=5cm]{Updated_plots/chibar_SHE.pdf}
    \caption{$\bar\chi$ for Heysham, Lowestoft, Newlyn and Sheerness (from top to bottom) for exceedances of the 0.9, 0.95, 0.975, 0.99 and 0.999 quantiles for various lags.}
    \label{fig::chibar}
\end{figure}

%\subsection{Modelling the Exceedance Probability with Tide and Day}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.49\textwidth]{Exprob_tide_av_HEY.pdf}
    \includegraphics[width=0.49\textwidth]{Updated_plots/Exprob_tide__averageLOW.pdf}
    \includegraphics[width=0.49\textwidth]{Updated_plots/Exprob_tide__averageNEW.pdf}        \includegraphics[width=0.49\textwidth]{Exprob_tide_av_SHE.pdf}
    \caption{Estimated trend in exceedance probability per month with respect to peak tide and day, averaged over day at Heysham (top left), Lowestoft (top right), Newlyn (bottom left) and Sheerness (bottom right). Trends for March (blue), June (black), September (cyan) and December (orange) are shown here.}
    \label{fig::exprobtide_av_all}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\textwidth]{Exprob_tide_MJSD_HEY.pdf}
    \includegraphics[width=0.75\textwidth]{Updated_plots/Exprob_tide_LOW_MJSD.pdf}
    \includegraphics[width=0.75\textwidth]{Updated_plots/Exprob_tide_NEW_MJSD.pdf}
    \caption{Estimated trend in exceedance probability per month with respect to peak tide and day at Heysham (top), Lowestoft (middle) and Newlyn (bottom). Darker points represent days later in the month, whilst lighter point represent days early in the month.}
    \label{fig::exprobtide_MJSD_all}
\end{figure}



%\subsection{Return Level Estimates}\label{extra_RLs}
%Here we show the return level estimates, monthly and annually, for all four scenarios listed in Section \ref{RLs}.

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.9\textwidth]{HEY_monmax_3x4_4.pdf}
%    \caption{Monthly return level estimates at Heysham for the proposed method (cyan), the current method (purple), intermediate solution I (blue) and intermediate solution II (magenta), compared with empirical estimates (red). We also show the highest astronomical tidal level (black dashed line).}
%    \label{HEY_monmax_4}
%\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=0.9\textwidth]{LOW_monmax_3x4_4.pdf}
%    \caption{Monthly return level estimates at Lowestoft for the proposed method (cyan), the current method (purple), intermediate solution I (blue) and intermediate solution II (magenta), compared with empirical estimates (red). We also show the highest astronomical tidal level (black dashed line).}
%    \label{LOW_monmax_4}
%\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=0.45\textwidth]{HEY_annmax_2.pdf}\includegraphics[width=0.45\textwidth]{LOW_annmax_4.pdf}
%    \caption{Annual return level estimates at Heysham (left) and Lowestoft (right) for the proposed method (cyan), the current method (purple), intermediate solution I (blue) and intermediate solution II (magenta), compared with empirical estimates (red). We also show the highest astronomical tidal level (black dashed line).}
%    \label{annmax_4}
%\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{Updated_plots/Mon_1x4_MJSD_allHEY.pdf} \\
    \includegraphics[width=0.8\textwidth]{Updated_plots/Mon_1x4_MJSD_allLOW.pdf} \\
    \includegraphics[width=0.8\textwidth]{Updated_plots/Mon_1x4_MJSD_allNEW.pdf} \\
    \includegraphics[width=0.8\textwidth]{Updated_plots/Mon_1x4_MJSD_allSHE.pdf} 
    \caption{Monthly sea level return level estimates for Heysham, Lowestoft, Newlyn and Sheerness (from top to bottom) in March, June, September and December, derived under \textit{baseline} (green), \textit{seasonal surge} (purple dashed), \textit{seasonal tide} (blue dashed), \textit{full seasonal} (cyan) methods and \textit{interaction} (red dot-dashed).}
    \label{fig::monmax_all_RL_NEW_1x4}
\end{figure}

\begin{figure}
    \centering 
    \includegraphics[width=0.49\textwidth]{Updated_plots/Ann_HEY_all.pdf}
    \includegraphics[width=0.49\textwidth]{Updated_plots/Ann_LOW_all.pdf} \\
    \includegraphics[width=0.49\textwidth]{Updated_plots/Ann_NEW_all.pdf}
    \includegraphics[width=0.49\textwidth]{Updated_plots/Ann_SHE_all.pdf} 
    \caption{Annual sea level return level estimates for Heysham (top left), Lowestoft (top right), Sheerness (bottom left) and Newlyn (bottom right) derived under \textit{current} (black dashed), \textit{baseline} (green), \textit{full seasonal} (cyan), \textit{interaction} (red dot-dashed) and \textit{temporal dependence} (orange dashed) methods, up to the 10,000 year level (right).}
    \label{fig::annmax_RL_NEW}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Updated_plots/Mappingannmax_HEY.pdf}
    \includegraphics[width=\textwidth]{Updated_plots/Mappingannmax_LOW.pdf}
    \includegraphics[width=\textwidth]{Updated_plots/Mappingannmax_NEW.pdf}
    \caption{PP plots for the transformed annual maximum sea levels to a uniform scale at Heysham (top), Lowestoft (middle) and Newlyn (bottom). These are transformed using the \textit{baseline} (left) and final (\textit{temporal dependence}) (centre) distribution function for the annual maxima, as well as the year specific final model (right). The black line shows the line of equality, $y=x$.}
    \label{fig::mapannmax_all}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{Updated_plots/Annmaxprob_RLs_HEY.pdf}
    \includegraphics[width=0.49\textwidth]{Updated_plots/Annmaxprob_RLs_NEW.pdf}
    \caption{Estimates of $\hat P_M(j;z_p)$ for all months $j=1,\ldots,12$ at Heysham (left) and Newlyn (right), for $p=1$ (dark green), 0.1 (green), 0.01 (cyan), 0.001 (blue), and 0.0001 (dark blue). The dashed dark green line is the empirical estimate of $P_M(j;z_p)$ for $p=1$.}
    \label{fig::Annmaxprob_HEYNEW}
\end{figure}


